Proverbs Run in Pairs: Evaluating Proverb Translation Capability of Large Language Model

Despite achieving remarkable performance, machine translation (MT) research remains underexplored in terms of translating cultural elements in languages, such as idioms, proverbs, and colloquial expressions. This paper investigates the capability of state-of-the-art neural machine translation (NMT) and large language models (LLMs) in translating proverbs, which are deeply rooted in cultural contexts. We construct a translation dataset of standalone proverbs and proverbs in conversation for four language pairs. Our experiments show that the studied models can achieve good translation between languages with similar cultural backgrounds, and LLMs generally outperform NMT models in proverb translation. Furthermore, we find that current automatic evaluation metrics such as BLEU, CHRF++ and COMET are inadequate for reliably assessing the quality of proverb translation, highlighting the need for more culturally aware evaluation metrics.

==> latex/2-background.tex <==
\section{Background}

==> tables/tab-annotator-instruction-proverb.tex <==
\begin{table*}[]
\centering
    \begin{tabular}{p{15cm}}
    \toprule
    \textsc{\textbf{Objective}} \\
    \midrule
    \makecell[tp{15cm}]{
    Your task is to analyse a given proverb in a language other than English and its provided English translation. You will evaluate the context dependency of the proverb, assess the accuracy of the translation, and suggest corrections if necessary.

- Please be as clear and concise as possible in your explanations.
- If you are unsure about the context dependency or translation accuracy, provide your best judgement and include a note explaining your reasoning.
- Use the space provided for each question to write your answers.
 \\\\
    \textit{\{ triplet \}}
    } \\
    \bottomrule
    \end{tabular}
    \caption{Proverb Translation Annotation Instruction}
% \vspace{-2mm}
\label{tab:question-prompt-fib}
\end{table*}

==> tables/tab-annotator-instruction-subtitles.tex <==
\begin{table*}[]
\centering
    \begin{tabular}{p{15cm}}
    \toprule
    \textsc{\textbf{Fill-in-blank Question}} \\
    \midrule
    \makecell[tp{15cm}]{
    I have a triplet extracted from a knowledge graph. The triplet is organized as (Subject, Relation, Object), which describes the relation between object and relation. Can you help me to generate a natural language sentence to describe this triplet as accurate as possible and replace Object with [MASK]? \\\\
    \textit{\{ triplet \}}
    } \\
    \bottomrule
    \end{tabular}
    \caption{Proverb Translation Annotation Instruction}
% \vspace{-2mm}
\label{tab:question-prompt-fib}
\end{table*}

==> tables/tab-proverb-filtered-stats.tex <==
\begin{table}[t]
\begin{center}
\scalebox{1}{
  \begin{tabular}{lrrr}
  \toprule
  \textbf{} &\multicolumn{1}{c}{\textbf{\#Proverbs}} & \multicolumn{1}{c}{\textbf{\#Pairs}} \\
  \midrule
  en -> bn  & 32 & 42 \\
  bn -> en & 5 & 8\\
  \midrule
  en -> de & 165 & 1540\\
  de -> en & 105 & 1129\\
  \midrule
  en -> id & 174 & 1214\\
  id -> en & 7 & 13\\
  \midrule
  en -> zh & 38 & 272\\
  zh -> en & 174 & 827\\
  \bottomrule                 
  \end{tabular}
 }
   % \vspace{-2mm}
   \caption{Filterd proverb translation data statistics}
   \label{tab:filtered-proverb}
   \end{center}
   % \vspace{-5mm}
\end{table}

